Compensation of Absorption Effects in Seismic Data

The frequency content of seismic data is changing with propagation depth due to intrinsic absorption. This implies that the higher frequencies are highly attenuated, thus leading to a loss in resolution of the seismic image. In addition, absorption anomalies, for example, caused by gas sands, will further dim the seismic reconstruction. It is possible to correct for such absorption effects by employing so called inverse Q filtering (IQF). This is a filtering technique that tries to restore the loss of the higher frequencies due to propagation. Newer developments within IQF can be regarded as a migration type of algorithm, and such classes of techniques are studied in this paper. As seismic waves travel through the earth, the visco-elasticity of the earth's medium will cause energy dissipation and waveform distortion. This phenomenon is referred to as seismic absorption. In explaining the propagation of seismic wave in a given medium we explore the relationship between the pressure and displacement stresses. Therefore, by introducing an absorption function into the stress and strain relationship we derived a non-linear wave equation. We, then, employed a layered earth model to solve the non-linear wave equation.

==> main-blx.tex <==
% Database for references
@article{wang2014absorption,
  title={Absorption-compensation method by l 1-norm regularization},
  author={Wang, Shoudong and Chen, Xiaohong},
  journal={Geophysics},
  volume={79},
  pages={V107--V114},
  year={2014},
  publisher={Society of Exploration Geophysicists}
}

@article{xue2019inverse,
  title={Inverse $\mathrm{Q}$ filtering via synchrosqueezed wavelet transform},
  author={Xue, Ya-Juan and Cao, Jun-Xing and Wang, Xing-Jian},
  journal={Geophysics},
  volume={84},
  pages={V121--V132},
  year={2019},
  publisher={Society of Exploration Geophysicists}
}

@article{zhao2018inverse,
  title={An inverse $\mathrm{Q}$ filtering approach based on a varying stabilization factor},
  author={Zhao, Yan and Mao, Ningbo},
  journal={Journal of Geophysics and Engineering},
  volume={15},
  pages={1269--1279},
  year={2018},
  publisher={Oxford University Press}
}
@article{rao2019stabilised,
  title={Stabilised inverse-$\mathrm{Q}$ filtering for seismic characterisation of carbonate reservoirs},
  author={Rao, Ying and Wang, Yanghua},
  journal={Journal of Geophysics and Engineering},
  volume={16},
  pages={190--197},
  year={2019},
  publisher={Oxford University Press}
}

@article{Ricker1953,
  title={The form and laws of propagation of seismic wavelets},
  author={Ricker, Norman},
  journal={Geophysics},
  volume={18},
  pages={10--40},
  year={1953},
  publisher={Society of Exploration Geophysicists}
}

@article{Kolsky1956,
  title={$\mathrm{LXXI}$. The propagation of stress pulses in viscoelastic solids},
  author={Kolsky, H},
  journal={Philosophical magazine},
  volume={1},
  pages={693--710},
  year={1956},
  publisher={Taylor \& Francis}
}

@article{Strick1967,
  title={The determination of $\mathrm{Q}$, dynamic viscosity and transient creep curves from wave propagation measurements},
  author={Strick, E},
  journal={Geophysical Journal International},
  volume={13},
  pages={197--218},
  year={1967},
  publisher={Oxford University Press}
}

@article{Wang2004,
  title={Modified $\mathrm{K}$olsky model for seismic attenuation and dispersion},
  author={Wang, Yanghua and Guo, Jian},
  journal={Journal of Geophysics and Engineering},
  volume={1},
  pages={187},
  year={2004},
  publisher={IOP Publishing}
}

@article{Futt1962,
  title={Dispersive body waves},
  author={Futterman, Walter I},
  journal={Journal of Geophysical Research},
  volume={67},
  pages={5279--5291},
  year={1962},
  publisher={Wiley Online Library}
}

@article{Kjart1979,
  title={Constant $\mathrm{Q}$-wave propagation and attenuation},
  author={Kjartansson, Einar},
  journal={Journal of Geophysical Research: Solid Earth (1978--2012)},
  volume={84},
  pages={4737--4748},
  year={1979},
  publisher={Wiley Online Library}
}

@article{Wang2002,
   author={Y. Wang},
   title={A Stable and Efficient Approach to Inverse $\mathrm{Q}$ Filtering},
   journal={Geophysics},
   volume={67},
   pages={1657--63},
   year={2002}
}


@article{Wang2006,
  title={Inverse $\mathrm{Q}$-filter for seismic resolution enhancement},
  author={Wang, Yanghua},
  journal={Geophysics},
  volume={71},
  pages={V51--V60},
  year={2006},
  publisher={Society of Exploration Geophysicists}
}


@article{LJGelius1987,
  title={Inverse $\mathrm{Q}$-filtering. A spectral balancing technique},
  author={Gelius, L J},
  journal={Geophysical prospecting},
  volume={35},
  pages={656--667},
  year={1987}
}


@article{Bickel1985,
   author={S. H. Bickel and R. R. Natarajan},
   title={Plane Wave $\mathrm{Q}$ Deconvolution},
   journal={Geophysics},
   volume={50},
   pages={1426--39},
   year={1985}
}


@article{Harg1991,
  title={Inverse $\mathrm{Q}$ filtering by Fourier transform},
  author={Hargreaves, Neil D and Calvert, Andrew J},
  journal={Geophysics},
  volume={56},
  pages={519--527},
  year={1991},
  publisher={Society of Exploration Geophysicists}
}

@article{Gjevik1976,
   title={An Attempt at the Inversion of Reflection DATA*},
  author={Gjevik, B and Nilsen, A and H{\"o}yen, J},
  journal={Geophysical prospecting},
  volume={24},
  pages={492--505},
  year={1976},
  publisher= {Wiley Online Library}
}

@book{Jaeger1962,
   title={Elasticity, fracture and flow with engineering and geological applications},
   author={Jaeger, John Conrad},
   publisher={Methuen \& Co. Ltd},
    year={1962},
   address={London, UK}
}

@article{Nilsen1978,
  title={Inversion of Reflection Data*},
  author={Nilsen, A and Gjevik, B},
  journal={Geophysical Prospecting},
  volume={26},
  pages={421--432},
  year={1978},
  publisher={Wiley Online Library}
}

@article{Horton1959,
  title={A loss mechanism for the Pierre shale},
  author={Horton, C W},
  journal={Geophysics},
  volume={24},
  pages={667--680},
  year={1959},
  publisher={Society of Exploration Geophysicists}
}

@book{Yilmaz2001,
   title={Seismic Data Analysis: Processing, inversion, and interpretation of seismic data},
   author={Yilmaz, {\"O}zdo{\u{g}}an},
   address = {Tulsa, USA},
   year={2001},
   publisher={Society of Exploration Geophysicists Tulsa}
}


@book{Aki2002,
   title={Quantitative Seismology},
  author={Aki, Keiiti and Richards, Paul G},
  year={2002},
  publisher={University Science Books},
  address = {Sausalito, CA}
}


@article{oliveira2013l1,
  title={L1 norm inversion method for deconvolution in attenuating media},
  author={Oliveira, S{\'e}rgio Adriano Moura and Lupinacci, Wagner Moreira},
  journal={Geophysical Prospecting},
  volume={61},
  pages={771--777},
  year={2013},
  publisher={Wiley Online Library}
}


@article{van2012bandwidth,
  title={Bandwidth enhancement: Inverse $\mathrm{Q}$ filtering or time-varying Wiener deconvolution},
  author={van der Baan, Mirko},
  journal={Geophysics},
  volume={77},
  pages={V133--V142},
  year={2012},
  publisher={Society of Exploration Geophysicists}
}


@article{montana2004compensating,
  title={Compensating for attenuation by inverse $\mathrm{Q}$ filtering},
  author={Monta\~{n}a, Carlos A and Margrave, Gary F},
  journal={CREWES Research Report},
  volume={16},
  year={2004}
}


@book{Kolsky1953,
   title={Stress Waves in Solids},
  author={Kolsky, H},
  year={1953},
  publisher={Clarendon Press},
  address={Oxford}
}


@book{wang2009seismic,
  title={Seismic Inverse $\mathrm{Q}$ Filtering},
  author={Wang, Yanghua},
  year={2009},
  publisher={John Wiley \& Sons}
}


@article{wang2004seismic,
  title={Seismic migration with inverse $\mathrm{Q}$ filtering},
  author={Wang, Yanghua and Guo, Jian},
  journal={Geophysical research letters},
  volume={31},
  pages={L21608--1},
  year={2004}
}


@article{cheng2011reflectivity,
  title={Reflectivity modeling for stratified anelastic media},
  author={Cheng, Peng and Margrave, Gary F},
  journal={CREWES Research Report},
  volume={23},
  year={2011}
}


@article{klimentos1995attenuation,
  title={Attenuation of P-and S-waves as a method of distinguishing gas and condensate from oil and water},
  author={Klimentos, Theodoros},
  journal={Geophysics},
  volume={60},
  pages={447--458},
  year={1995},
  publisher={Society of Exploration Geophysicists}
}


@article{mitchell1987effect,
  title={Effect of low $\mathrm{Q}$ sediments and crustal $\mathrm{Q}$ on Lg attenuation in the United States},
  author={Mitchell, Brian J and Hwang, HJ},
  journal={Bulletin of the Seismological Society of America},
  volume={77},
  pages={1197--1210},
  year={1987},
  publisher={The Seismological Society of America}
}


@article{robinson1979technique,
  title={A technique for the continuous representation of dispersion in seismic data},
  author={Robinson, John C},
  journal={Geophysics},
  volume={44},
  pages={1345--1351},
  year={1979},
  publisher={Society of Exploration Geophysicists}
}

